Active Learning for Accurate Estimation of Linear Models

We explore the sequential decision making problem where the goal is to estimate uniformly well a number of linear models, given a shared budget of random contexts independently sampled from a known distribution. The decision maker must query one of the linear models for each incoming context, and receives an observation corrupted by noise levels that are unknown, and depend on the model instance. We present Trace-UCB, an adaptive allocation algorithm that learns the noise levels while balancing contexts accordingly across the different linear functions, and derive guarantees for simple regret in both expectation and high-probability. Finally, we extend the algorithm and its guarantees to high dimensional settings, where the number of linear models times the dimension of the contextual space is higher than the total budget of samples. Simulations with real data suggest that Trace-UCB is remarkably robust, outperforming a number of baselines even when its assumptions are violated.

==> inputs/baselines.tex <==
% !TEX root = ../pure_exploration_gaussian_bandits.tex

\section{Baselines}
\label{baselines}
%Main points:
%\begin{enumerate}
%\item Intuition: sources of error. [1 paragraph]
%\item Intuition: types of scenarios. [1 paragraph]
%\item Random Sampling. [2 paragraphs]
%\item Optimal Static Allocation. [2 paragraphs]
%\item Context Free Algorithm [2 paragraphs]
%\end{enumerate}
In this section, we first discuss a few key observations regarding the problem, and different scenarios.
Then, we present three baseline algorithms: the optimal static allocation, random allocation, and a context-free algorithm that was introduced in \cite{carpentier2011upper}.

The loss function we minimize is the maximum expected squared prediction error over arms.
For a fixed arm, say $i$, the prediction error ---assuming an unbiased estimator--- comes from two different sources.
The first one is the fact that the $\Y$ measurements are noisy.
The strength of the noise is controlled by $\sigma_i^2$, which is unknown.
Clearly, the larger $\sigma_i^2$ is, the more observations will be required for the same accuracy level.
On the other hand, the \emph{diversity} of contexts also matters.
It would be a terrible idea for the MOOC platform mentioned in the introduction to estimate the History parameters by performing a hundred exams on the very same student (same context).
We say contexts are balanced when $\X^T\X$ is well conditioned.
Therefore, a good algorithm needs to take care of both aspects.

There are two extreme scenarios regarding the contribution from both sources of error.
First, if the number of contexts $T$ is relatively large, one can expect contexts falling in each arm to balance themselves automatically (under a sensible algorithm).
In this case, the difference in the $\sigma_i^2$'s will mostly determine the number of times each arm should be pulled.
Second, when the dimension of the space $d$ or the number of arms $m$ grow large with respect to $T$,  then balancing contexts becomes critical, and can drive the final prediction error. 
The $\sigma_i^2$'s are less relevant in this scenario.

Thus, good algorithms should smoothly handle both cases.
Keeping this in mind, we discuss a few natural baselines.

We start by describing the optimal static allocation under the assumption that the $\sigma_i^2$'s are known.
A static algorithm decides the number of pulls per arm before the starting of the process, and it does not take into account contexts.

When the number of pulls for each arm $i$ is deterministic, and equal to $k_i$, Theorem 1.1 in the Appendix shows that
\begin{equation}\label{eq_exp_loss_formula}
\mathbf{L} = \max_{i \in [m]} \E \left[ \| \beta_i - \hat\beta_i \|^2_{\Sigma} \right] = \max_{i \in [m]} \E \left[ \frac{\sigma_i^2}{k_i} \mathrm{Tr}(\Sigma \hat\Sigma_{k_i}^{-1}) \right],
\end{equation}
where $\hat\Sigma_{k_i}^{-1} := (\X_i^T \X_i / k_i)^{-1}$ is the empirical inverse covariance matrix for arm $i$ after pulling data $\X_i$.
In addition, if contexts are Gaussian, there is a closed-form expression for the trace in \eqref{eq_exp_loss_formula}, leading to a closed-form solution for the optimal number of pulls per arm:
\begin{equation}\label{eq_opt_stat_alloc}
k_i^* = \frac{\sigma_i^2}{\sum_j \sigma_j^2} \ T + (d+1) \ \left( 1 - \frac{\sigma_i^2}{\bar{\sigma}^2} \right),
\end{equation}
where $\bar{\sigma}^2 := \sum_j \sigma_j^2 / m$ is the mean error variance.
% See Theorem 1.1 in the Appendix.
Note that the allocation is proportional to the $\sigma_i^2$'s, plus a linear contribution in $d$ that requires more pulls for low-variance arms; in particular, those whose $\sigma_i^2$ is below the mean $\bar\sigma^2$.

The expected loss of the optimal static allocation $\mathbf{L}^*$ is
\begin{equation}\label{eq_opt_stat_loss}
\mathbf{L}^* = \sum_j \sigma_j^2 \ \frac{d}{T} + O \left( \left( \sum_j \sigma_j^2 \right) m \left( \frac{d}{T} \right)^2 \right),
\end{equation}
as derived in Theorem 1.2 in the Appendix.
% Thus, no arm is first order bottleneck.
As also shown in the theorem, $\mathbf{L}^* \ge (\sum_j \sigma_j^2) d / T$.
This allocation can't be used in practice, however, as the $\sigma_i^2$'s are unknown.
We choose the optimal static allocation as our regret benchmark as it does not face the exploration-exploitation trade-off because $\sigma_i^2$'s and $\F$ are both known.

The most basic practical approach is random sampling.
The algorithm simply pulls every arm equally often, or $\approx T / m$ times, and it does not look at the current context.
The performance of the algorithm will be poor in general, except when $\sigma_{\max}^2 \approx \sigma_{\min}^2$.
The bottleneck for random sampling is the arm with the largest $\sigma_{i}^2$, which requires the most pulls.
The loss of random sampling $\mathbf{L}_{\mathrm{RS}}$ is given by
\begin{equation}\label{eq_rs_loss}
\mathbf{L}_{\mathrm{RS}} = \sigma_{\max}^2 m \ \frac{d}{T} + o\left( \frac{1}{T} \right). 
\end{equation}
Note the difference with respect to the leading term in \eqref{eq_opt_stat_loss}.

Another baseline is the UCB-type algorithm presented in \cite{carpentier2011upper} to solve the context-free problem \cite{antos2008active}.
The algorithm greedily pulls arms according to an upper bound on the estimated current prediction error for each arm $i$, which is based on confidence intervals for each $\sigma_i^2$.
We extend this idea to the contextual case by updating the estimated prediction error to include the contribution of the contexts seen so far at each arm.









==> inputs/high_dims.tex <==
% !TEX root = ../pure_exploration_gaussian_bandits.tex

\section{High Dimensional Setting}
\label{sec:high-dim}
%Main points:
%\begin{enumerate}
%\item Motivation: why do we study HDim? [1 paragraph]
%\item High Dim Setting [1 paragraph]
%\item Intuition: what we need to change from TraceUCB. [1 paragraph]
%\item Lasso Recovery: Intro and Lit Review. [1 paragraph]
%\item Description of HighDTraceUCB + pseudocode. [2 paragraphs]
%\item High Probability Guarantees [2 paragraphs]
%\end{enumerate}
%%% motivation
High-dimensional linear regression models are remarkably common in practice.
Companies tend to record a large number of features of their customers, and feed them to their prediction models. There are also cases in which the number of problem instances under consideration $m$ is large, e.g.,~too many courses in the MOOC example described in the introduction. Unless the horizon $n$ is still proportionally large w.r.t. $md$, these scenarios require special attention. In particular, algorithms like \traceucb that adaptively use contexts in their allocation strategy become more robust than their context-free counterparts. 

A natural assumption in such scenarios is {\em sparsity}, i.e.,~only a small subset of features are relevant to the prediction problem at hand (have non-zero coefficient). In our setting of $m$ problem instances, it is often reasonable to assume that these instances are related to each other, and thus, it makes sense to extend the concept of sparsity to {\em joint sparsity}, i.e.,~a sparsity pattern across the instances. Formally, we assume that there exists a $s \ll d$ such that
%
\begin{equation}
|S| \stackrel{\Delta}{=} | \cup_{i \in [m]} \text{supp}(\beta_i) | = s,
\end{equation}
%
where $\text{supp}(\beta_i) = \{ j \in [d] : \beta_i^{(j)} \neq 0 \}$ denotes the support of the $i$'th problem instance. A special case of joint sparsity is when $| \text{supp}(\beta_i) | \approx s$, for all $i$, i.e.,~most of the relevant features are shared across the instances.


%Intuitively, when $n$ becomes larger and larger, the problem becomes easier and easier, and sensible algorithms should lead to very accurate estimates for all arms.
%On the other hand, in practical applications, it is often the case that $d$ ends up being quite large; for example, data scientists tend to add as many features as available, and, sometimes, even non-linear transformations and interactions are included.
%In addition, in some cases the number of alternatives $m$ may be extremely large.
%Unless the budget of pulls $n$ is still proportionally large, these situations require a more careful approach.
%In particular, we may not be even able to pull each arm $d+1$ times, the first step of \traceucb.
%
%A natural assumption in those scenarios is that of \emph{sparsity}: some of the contextual dimensions do \emph{not} matter for the outcome.
%The MOOC platform described in the introduction may log the local time at which each student decided to register for the course.
%Even though it seems unlikely that such information is helpful for predicting the performance of the student in a Math exam, the engineer could easily add it to the model (say, whether it was in the morning, afternoon or evening).
%In a high-dimensional setting where pulls are scarce, the algorithm should quickly learn whether local time at registration is or not relevant, and in the latter case, discard it.
%
%Moreover, when learning about $m$ related alternatives, we think it is reasonable to link their sparsity.
%We assume \emph{joint} sparsity across arms; the sparsity pattern of all arms agree on a large proportion of the non-zero elements, while each arm may still have a few unique non-zero components. 
%
%Formally, we assume that there exists $s \ll d$ such that
%\begin{equation}
%|S| := | \cup_{i \in [m]} \text{supp}(\beta_i) | = s,
%\end{equation}
%where $\text{supp}(\beta_i) = \{ j \in [d] : \beta_{ij} \neq 0 \}$ denotes the support of arm $i$. 
%The main regime of interest is that where $| \text{supp}(\beta_i) | \approx s$ for all $i$, so most of the non-zero components are shared.

In this section, we focus on the scenario where $dm > n$. When we can only allocate a small (relative to $d$) number of contexts to each problem instance, proper balancing of contexts become extremely important, and thus, the algorithms that do not take into account context in their allocation are destined to fail. Although \traceucb has the advantage of using context in its allocation strategy, it still needs to quickly discover the relevant features (those in the support) and only use those in its allocation strategy.

This motivates a two-stage algorithm, we call it \sparsetraceucb, whose pseudocode is in Algorithm~\ref{alg:sparse_trace_ucb} in Appendix~\ref{app:high.dimensions}. In the first stage, the algorithm allocates contexts uniformly to all the instances, $L$ contexts per instance, and then recovers the support. In the second stage, it relies on the discovered support $\wh S$, and applies the standard \traceucb to all the instances, but only takes into account the features in $\wh S$. Note that $L$ should be large enough that with high probability, support is exactly discovered, i.e., $\wh S = S$.

There exists a large literature on how to perform \emph{simultaneous} support discovery in jointly sparse linear regression problems~\cite{negahban2011simultaneous, obozinski2011support, wang2013block}. Most of these algorithms minimize the regularized empirical loss
%
\begin{equation*}\label{opt_problem}
\min_{\mathrm{M} \in \R^{d \times m}} \frac{1}{k} \sum_{i=1}^m \| \Y_i - \X_i \ \mathrm{M}[,i] \|^2 + \lambda \ \| \mathrm{M} \|,
\end{equation*}
%
where $k$ is the number of samples per problem, $\mathrm{M}$ be the matrix whose $i$'th column is $\mathrm{M}[,i] = \hat{\beta}_i$, $\X_i \in \R^{k \times d}$, and $\Y_i = \X_i \beta_i + \epsilon_i$. In particular, they use $l_a/l_b$ block regularization norm, i.e.,~$\| \mathrm{M} \|_{l_a/l_b} = \| v \|_{l_a}$, where $v_i = \| \mathrm{M}[i,] \|_{l_b}$ and $\mathrm{M}[i,]$ is the $i$'th row of $\mathrm{M}$. 

The \sparsetraceucb algorithm uses the $l_1/l_2$ block regularization Lasso algorithm~\cite{wang2013block}, which is an extension of the algorithm in~\cite{obozinski2011support}, for its support discovery stage.

%under suitable assumptions, see C1-C5 in Appendix \ref{app:high.dimensions}.

%As we explained in previous sections, at time $t$ and for each arm $i$, \traceucb takes into account the contribution of contexts $\X_{i,t}$ to the current estimation error.
%However, if we knew that some of the components $j$ are such that $\beta_{ij} = 0$, then we could simply ignore the components altogether, and reduce the dimensionality of the space for arm $i$.
%The key observation is that we want to do this as soon as possible, as, otherwise, we would be making allocation decisions based on a score that partly relies on something that does not matter.
%Of course, in practice we do not know whether $\beta_{ij} = 0$ or not, and we need to collect enough data to make sure we are not actually discarding relevant dimensions.
%
%This motivates a two-stage algorithm.
%In the first stage, we pull every arm equally often, say $L$ times, and at the end we jointly recover the support.
%In the second stage, we rely on the support that was recovered in the previous stage.
%Then, we apply the standard \traceucb to all arms, but taking into account only those dimensions that are in the support (all other components are ignored).
%Note that we need to collect enough data in the recovery stage, so that with high probability the recovery is exact.

%There is a large literature on how to perform \emph{simultaneous} support recovery in sparse settings for multiple regressions \cite{negahban2011simultaneous, obozinski2011support, wang2013block}.
%Let $\mathrm{M}$ be the matrix whose $i$-th column is $\mathrm{M}^{(i)} = \hat{\beta}_i$.
%Assume $k$ observations per arm; then many algorithms minimize the regularized empirical loss
%\begin{equation}\label{opt_problem}
%\min_{\mathrm{M} \in \R^{d \times m}} \frac{1}{k} \sum_{i=1}^m \| \Y_i - \X_i \ \mathrm{M}^{(i)} \|^2 + \lambda \ \| \mathrm{M} \|,
%\end{equation}
%where $\Y_i = \X_i \beta_i + \epsilon_i$, $\X_i \in \R^{k \times d}, \Y_i \in \R^k$, $\beta_i \in \R^d$.
%
%In particular, the $l_a/l_b$ block regularization norm is
%\begin{equation}
%\| \mathrm{M} \|_{l_a/l_b} = \| v \|_a,
%\end{equation}
%where $v_i = \| \mathrm{M}_i \|_b$, and $\mathrm{M}_i$ is the $i$-th row of $\mathrm{M}$.

We can now extend the guarantees of Theorem \ref{thm_high_prob} to the high dimensional case with joint sparsity, assuming $s$ is known.
\begin{theorem}\label{thm_high_prob_sparse}
Let $\delta_1 > 0$.
Assume $\| \beta_i \|_2 \le Z$ for all $i$, for some $Z > 0$, and assume the parameters $(n, d, s, \beta_i, \Sigma)$ satisfy conditions \textbf{C1} to \textbf{C5} in \cite{wang2013block}.
Let $\psi$ be the sparsity overlap function defined in \cite{obozinski2011support}.
If $L > 2(1+v) \ \psi \ \log(d-s) {\rho_u(\Sigma^{(1:m)}_{S_C S_C | S})}/{\gamma^2}$ for some constant $v > 0$, and $n-Lm \ge (s+1)m$, then, with probability at least $1 - \delta_1 - \delta_2$, $\hat{\mathbf{L}}$ is at most
\begin{equation}
\frac{\sum_j \sigma_j^2}{n-Lm} \left( s + 2 \log \frac{3m}{\delta_1} \right) +  \frac{2c}{\sqrt{\sigma_{\min}^2}}   \left( \frac{s \sum_j \sigma_j^2}{n - Lm} \right)^{3/2} + o \left( z \right),
\end{equation}
where $c \le 2\left(1 + \sqrt{2 \log ({12mn}/{\delta_1}) / s} \right)$
and we defined $\delta_2 = m \exp(-c_0 \log s) + \exp(-c_1 \log(d-s))$ for positive constants $c_0, c_1 > 0$, and $z = \left( {s}/{(n-Lm)} \right)^{3/2}$.
\end{theorem}
The exact technical assumptions and the proof are given and discussed in Appendix \ref{app:high.dimensions}.
We simply combine the high-probability results of Theorem \ref{thm_high_prob}, and the high-probability support recovery of Theorem 2 in \cite{wang2013block}.
Corollary~\ref{cor:high_dim_traceucb} studies the regime of interest where the support overlap is complete, $n = C_1 \ m s \log d \ll md$ for $C_1 > 0$, and $L = C_2 \ s \log d$, for $C_1 - C_2 > 0$ (see Appendix \ref{app:high.dimensions}).
%\begin{corollary}
%Under the assumptions of Theorem \ref{thm_high_prob_sparse}, let $\delta_1 > 0$, assume $n = C_1 \ m s \log d$, the support of all arms are equal, and set $L = C_2 \ s \log d$, for $\bar{C} := C_1 - C_2 > 0$.
%Then, with probability at least $1 - \delta_1 - \delta_2$, $\hat{\mathbf{L}}$ is at most
%\begin{equation}
%\frac{\sum_j \sigma_j^2}{\bar{C} ms \log d} \left( s + 2 \log \frac{3m}{\delta_1} \right) +  \frac{2c}{\sqrt{\sigma_{\min}^2}}   \left( \frac{\sum_j \sigma_j^2}{\bar{C} m \log d} \right)^{3/2} + o \left( z \right)
%\end{equation}
%where $c \le 2\left(1 + \sqrt{2 \log ({12mn}/{\delta_1}) / s} \right)$ and we defined $\delta_2 = m \exp(-c_0 \log s) + \exp(-c_1 \log(d-s))$ for constants $c_0, c_1 > 0$, and $z = \left( \bar{C} m \log d \right)^{-3/2}$.
%\end{corollary}


